From Past to Future: Rethinking Eligibility Traces

In this paper, we introduce a fresh perspective on the challenges of credit assignment and policy evaluation. First, we delve into the nuances of eligibility traces and explore instances where their updates may result in unexpected credit assignment to preceding states. From this investigation emerges the concept of a novel value function, which we refer to as the \emph{bidirectional value function}. Unlike traditional state value functions, bidirectional value functions account for both future expected returns (rewards anticipated from the current state onward) and past expected returns (cumulative rewards from the episode's start to the present). We derive principled update equations to learn this value function and, through experimentation, demonstrate its efficacy in enhancing the process of policy evaluation. In particular, our results indicate that the proposed learning approach can, in certain challenging contexts, perform policy evaluation more rapidly than TD($\lambda$) -- a method that learns forward value functions, $v^\pi$, \emph{directly}. Overall, our findings present a new perspective on eligibility traces and potential advantages associated with the novel value function it inspires, especially for policy evaluation.

==> literature.tex <==
\cite{zhang2020learninga}
The paper answers question like how much fuel do expect the car to have given it is at B at time "t". The agent needs to have some form of retrospective knowledge with reverse GVF's. trained using Reverse RL.  Utility of method is shown for \textbf{Representation Learning} and \textbf{Anomaly Detection}.

The paper starts by talking about a reverse return which is similar  to our definition $\bar{G}_t = R_{t-1} + \gamma(S_{t-1})\bar{G_{t-1}}$. The paper provides a bellman equation for the above function and shows that the value function exists and can indeed be learned through stocashtic approximation approach. The paper also introduces a disrtibutional variant of the above in order to decide when the previous return observed might not lie in the disrtibution that it usually is. 
\begin{itemize}
    \item Provides theory of convergence and assumptions and also existence of the value function $\bar{v}(s) = \EE{}{\bar{G_t} | S_t = s}$, in the limit of $t \rightarrow \infty$. 
    \item They also have an off policy version of the reverse TD version which relies on actually using the state density estimation $d_\pi, d_\mu$ from the behaviour and target policies under consideration. 
    \item Proposition 1 : Defines the convergence of Reverse TD assuming lineary independent features and columns of matrices and also talks about a TD$(\lambda)$ version. 
    \item The experiments are provided on the case of anomaly detection for a small microdrone environment as well as reacher for a anomalous reward detection. Another experiment is shown for Representation Learning where they adapt previous work on \cite{veeriah2019discovery} automatically discovered GVF's act as good aux tasks for representation learning.They show the same actually happens for the reverse GVF's as well as compared to some other aux tasks. 
    \item One important part of the related works, \cite{morimura2010derivatives} shows that if the initial distribution $\mu_0$ is changed to $d_\pi$, we can redefine the transition matrix and policy such that we can get an equivalent MDP which flows in the reverse diretion to this other MDP. The important thing to notice is that a trajectory $\{ S_0, A_0, .... , S_k\}$ from the original MDP following $\pi$ can be thought of as a trajectory $\{ S_k, A_k, .... , S_0\}$ from the new MDP (reverse). These things are acceptable only in the on policy case, as we require acess to $d_\pi$ for the case of off-policy learning. 
\end{itemize}
% \lb{comment below out for now}
% \cite{jiang2022learning}

% \cite{zhang2021deep}

% \cite{lyle2022learning}

% \cite{lyle2021on}

% \cite{ghosh2020representations}

% \cite{xu2017natural} 

==> related.tex <==
\paragraph{Backward Temporal Difference Model}
Backward TD model, or termed reverse TD model~\cite{{doina:chelu2020forethought,zhang2020learninga}}


% 1. Definition:
Backward Temporal Difference (TD) Learning is an approach in Reinforcement Learning (RL) that incorporates ``hindsight'' or ``retrospective'' knowledge into credit assignment. It generally works by considering the impact of a current decision on future states, not just on the immediate reward, thereby assigning credit for actions based on future consequences, moving from the future state to the current state.
% 2. Importance:


% 3. Difference with Forward TD Learning:
Forward TD learning models use a "forward-view", where updates are made based on the expected future rewards from the current state-action pairs, and the learning propagates from the current state to the future state. On the other hand, Backward TD Learning employs a "backward-view". It estimates the value of the current state by looking at the actual future states (not just the expected ones), thereby propagating learning from the future state back to the current state.

% 4. Major Achievements:
Several advancements have been made in the field of backward TD learning:
Chelu, Precup, and van Hasselt (2020) discussed the importance of both forethought and hindsight in credit assignment, showing how both views can help improve the performance of RL algorithms.  
Wang et al. (2021) proposed an offline RL approach that utilizes reverse model-based imagination, demonstrating the potential of backward TD learning in offline settings where data collection is expensive or risky.   
Xu et al. (2022) developed a unifying framework for off-policy general value function evaluation, which incorporated backward TD learning to improve off-policy learning.   
Park and Wong (2022) demonstrated robust imitation from a few demonstrations using a backward model, showcasing the value of backward TD learning in imitation learning scenarios.   
Zhang, Veeriah, and Whiteson (2020) presented the concept of learning retrospective knowledge with reverse reinforcement learning, further emphasizing the importance of incorporating hindsight in RL algorithms.

\textcolor{red}{Perhaps also reference Chris Nota's work on posterior value functions.}
   
Overall, backward TD learning is a promising approach in reinforcement learning, offering more efficient credit assignment and learning in complex environments.




\paragraph{Stability and Convergence of TD($\lambda$)}
\lb{The focus of the paper is not the stability or convergence of TD($lambda$), but on the question: When and why backward TD($\lambda$) performs better than forward TD($\lambda$)? So not sure if it is worthwhile to do surveys on Stability and Convergence of TD($lambda$).}

==> related_work_extra.tex <==

\section{Literature Review}

\subsection{TD($\lambda$) for Deep RL}

The successful application of eligibility traces has been historically associated with linear function approximation \citep{sutton1984temporal, sutton2018introduction}. The update rules for eligibility traces, explicitly designed for linear value functions, encounter ambiguities when extended to nonlinear settings. As the RL community gravitated towards non-linear function approximators—chiefly due to the rise of deep RL—the interpretations of these rules for such approximators became multi-faceted and no single interpretation emerged as dominant. Several attempts to adapt traces for deep RL \cite{tesaurio1992practical,elfwing2018sigmoid} faced challenges, largely owing to the pervasive use of experience replay in modern deep RL \cite{mnih2015human}. Still, traces have found some utility in methods such as advantage estimation \cite{schulman2017proximal}. One notable interpretation, put forward by \cite{hasselt2020expected}, applies linear traces to the penultimate layer of a deep value function approximator, maintaining a linear view for the final layer.

\subsection{Backward Temporal Difference Models}

Backward Temporal Difference (TD) Learning offers a fresh perspective to RL by integrating `hindsight' into the credit assignment process. Unlike traditional forward-view TD learning, which bases updates on expected future rewards from present decisions, backward TD works retrospectively, estimating present values from actual future outcomes. This shift to a 'backward-view' has spurred significant advancements. Chelu et al. \cite{doina:chelu2020forethought} underscored the pivotal roles of both foresight and hindsight in RL, illustrating their combined efficacy in algorithmic enhancement. Wang et al. \cite{wang2021reverse} leveraged backward TD for offline RL, illuminating its potential in settings where data collection proves challenging. Further, the prowess of backward TD learning in imitation learning was highlighted by Park and Wong \cite{park2022backward}. \cite{zhang2020learninga} reinforced the need for retrospective knowledge in RL, cementing the pertinence of the backward view. \textcolor{red}{Additional references, such as Chris Nota's work, can further enrich this discussion.}

\subsection{Auxiliary Rewards for Value Learning}

Auxiliary tasks, when incorporated into RL, often act as catalysts, refining the primary task's learning dynamics. Such tasks span various functionalities—next-state prediction, reward forecasting, representation learning, and policy refinement, to name a few \cite{lin2019adaptive,rafiee2022makes}. The "Unsupervised Auxiliary Tasks" framework proposed by Jaderberg et al. \cite{jaderberg2016reinforcement} serves as testament to the enrichment auxiliary tasks bring to feature representations, mutually benefiting both main and auxiliary tasks. Another significant contribution, "Curiosity-Driven Exploration" by Pathak et al. \cite{pathak2017curiosity}, places emphasis on the agent's innate curiosity, devising auxiliary tasks that champion state exploration novelty, substantially augmenting the agent's exploration and adaptability.






\begin{enumerate}
\item TD($\lambda$) for deep RL
\item Backward/Forward TD models
\item Auxiliary Rewards for Value learning
\end{enumerate}

Although traces have enjoyed major success, but almost all the application and theory of traces has been limited to the case where the value function is linear in the parameters \citep{sutton1984temporal, sutton2018introduction}. This is because the update rules for traces are only defined for linear value functions. However, nowdays scaling up RL moslty entails using a non linear function approximator (i.e., Deep RL), for which case the update rules of traces although define can have multiple interpretation with no single one being the intended one. \todo{Not sure about this line}. Previous applications of traces to deep RL \cite{tesaurio1992practical,elfwing2018sigmoid} has mostly been limited partly due to the success of  replay memory \cite{mnih2015human}, although popular methods \cite{schulman2017proximal} still make of $\lambda$ returns for advantage estimation .\cite{hasselt2020expected} has provided one interpretation of traces, where the penulimate layer is treated as the representation and hence a linear trace is maintained for the weights on the last layer of the value function network. 

Given the context above, it is not as if traces have not been applied for neural networks previously (nonlinear FA). Eligibility traces have been successfully applied in  \cite{tesaurio1992practical, elfwing2018sigmoid, javed2023online}  to train their function, and as mentioned above with a slow enough change the traces should work fine. Another reason for the sparse adoption of traces is because of the success of experience replay \cite{mnih2015human} which is not applicable to the idea of traces, as one only stores single transitions rather than full episodes which are required to perform TD($\lambda$). \citep{daley2018efficient}  had shown a way to cache $\lambda$ returns while storing the transition in replay buffer to implement some form forwards view, with some added complexity, but the functional compatibility still exists. 


The stability of TD($\lambda$), explicitly TD(0) has been previously discussed extensively for non-linear function approximation in 

%% v1
% RL with auxiliary tasks has gained significant attention as a promising approach to enhance the learning performance of the main task. By incorporating additional objectives alongside the primary task, the agent can acquire a richer understanding of the environment and accelerate its learning process. Auxiliary tasks are often used for predicting the next state, predicting rewards, learning representations, and policy improvement~\cite{lin2019adaptive,rafiee2022makes,hernandez2019agent,kartal2019terminal,tongloy2017asynchronous,bellemare2019geometric,veeriah2018many,yarats2021improving}. 

% We briefly sketch some landmark work in this research direction. \cite{jaderberg2016reinforcement} proposed the "Unsupervised Auxiliary Tasks" framework, demonstrating that auxiliary tasks can lead to better feature representations, benefiting both the main and auxiliary objectives.
% \cite{pathak2017curiosity} presented "Curiosity-Driven Exploration" (Curiosity), where the agent is driven by the curiosity to explore its environment, learning auxiliary tasks that encourage novel states. This approach significantly improved the agent's exploration and generalization capabilities.

%%% v2
The integration of auxiliary tasks in Reinforcement Learning (RL) has garnered considerable attention as a promising strategy to enhance the learning performance of the primary task. By introducing supplementary objectives in conjunction with the main task, the agent gains a more comprehensive understanding of the environment, thereby expediting its learning process. These auxiliary tasks encompass diverse functions, such as next-state prediction, reward prediction, representation learning, and policy enhancement \cite{lin2019adaptive,rafiee2022makes,hernandez2019agent,kartal2019terminal,tongloy2017asynchronous,bellemare2019geometric,veeriah2018many,yarats2021improving}. Jaderberg et al. \cite{jaderberg2016reinforcement} proposed the "Unsupervised Auxiliary Tasks" framework, demonstrating that auxiliary tasks contribute to better feature representations, benefiting both the primary and auxiliary objectives. Additionally, Pathak et al. \cite{pathak2017curiosity} presented "Curiosity-Driven Exploration" (Curiosity), a novel approach where the agent's exploration is propelled by curiosity, encouraging the learning of auxiliary tasks that foster novel state exploration. This approach exhibits a significant enhancement in the agent's exploration and generalization capabilities.



\paragraph{Backward Temporal Difference Model}
Backward TD model, or termed reverse TD model~\cite{{doina:chelu2020forethought,zhang2020learninga}}


% 1. Definition:
Backward Temporal Difference (TD) Learning is an approach in Reinforcement Learning (RL) that incorporates ``hindsight'' or ``retrospective'' knowledge into credit assignment. It generally works by considering the impact of a current decision on future states, not just on the immediate reward, thereby assigning credit for actions based on future consequences, moving from the future state to the current state.
% 2. Importance:


% 3. Difference with Forward TD Learning:
Forward TD learning models use a "forward-view", where updates are made based on the expected future rewards from the current state-action pairs, and the learning propagates from the current state to the future state. On the other hand, Backward TD Learning employs a "backward-view". It estimates the value of the current state by looking at the actual future states (not just the expected ones), thereby propagating learning from the future state back to the current state.

% 4. Major Achievements:
Several advancements have been made in the field of backward TD learning:
Chelu, Precup, and van Hasselt (2020) discussed the importance of both forethought and hindsight in credit assignment, showing how both views can help improve the performance of RL algorithms.  
Wang et al. (2021) proposed an offline RL approach that utilizes reverse model-based imagination, demonstrating the potential of backward TD learning in offline settings where data collection is expensive or risky.   
Xu et al. (2022) developed a unifying framework for off-policy general value function evaluation, which incorporated backward TD learning to improve off-policy learning.   
Park and Wong (2022) demonstrated robust imitation from a few demonstrations using a backward model, showcasing the value of backward TD learning in imitation learning scenarios.   
Zhang, Veeriah, and Whiteson (2020) presented the concept of learning retrospective knowledge with reverse reinforcement learning, further emphasizing the importance of incorporating hindsight in RL algorithms.

\textcolor{red}{Perhaps also reference Chris Nota's work on posterior value functions.}
   
Overall, backward TD learning is a promising approach in reinforcement learning, offering more efficient credit assignment and learning in complex environments.




\paragraph{Stability and Convergence of TD($\lambda$)}
\lb{The focus of the paper is not the stability or convergence of TD($lambda$), but on the question: When and why backward TD($\lambda$) performs better than forward TD($\lambda$)? So not sure if it is worthwhile to do surveys on Stability and Convergence of TD($lambda$).}
